Cooperation and Cognition in Social Networks

Social networks can sustain cooperation by amplifying the consequences of a single defection through a cascade of relationship losses. Building on Jackson et al. (2012), we introduce a novel robustness notion to characterize low cognitive complexity (LCC) networks - a subset of equilibrium networks that imposes a minimal cognitive burden to calculate and comprehend the consequences of defection. We test our theory in a laboratory experiment and find that cooperation is higher in equilibrium than in non-equilibrium networks. Within equilibrium networks, LCC networks exhibit higher levels of cooperation than non-LCC networks. Learning is essential for the emergence of equilibrium play.

==> prev_comments.tex <==
Model

%\emph{Edo: some comments on this section:
%\begin{itemize}
%    \item we should have 3 propositions for i) rnp, ii) sq and iii) CS. proofs will be in appendix (where necessary give it is a reduced form of JRT) but we should introduce enough "machinery" for a formal statement of the proposition. each proposition should be followed by one paragraph that give the intuition about the result/proof (when necessary, for sure for the cs networks)
%    \item for discussion: i think initial set-up should not be about deleting links (as in experiment) but, like JRT, random draw of a link for favour. the way it is written I am not sure they are strategically the same, eg if I am the peripheral node of a 3-triangle I may want to delete the link with the center rather than the other peripheral node if I see that the center has a missing link b/c that may give me information about the center tendency to delete links
%    \item we still need to be more formal, eg def 2 talks about strategies but these have not been defined formally in the model set-up
%\end{itemize}}

%Comments to the draft of the section:
%\begin{itemize}
%    \item in general it needs to be more concise and formal 
%    \item start from the model that we use without mentioning or relying on any prior knowledge from the jackson model (ie assume the reader has never heard/seen the jackson model and does not need to know at this stage)
%    \item after our model has presented then you point the key simplifications from the jackson one
%    \begin{itemize}
%        \item  (to be discussed: as far as I remember links are exogenous in jackson too)
%        \item to be discussed: keep the poisson formulation for us as well? the fact we do not have it in the experiment is just an implementation 
%    \end{itemize}
%    \item minor point: introduce references (ie to social quilts paper and i'd call it with the 3-letter acronym of the authors rather than jackson model)
%\end{itemize}


%For the purposes of the modified model to adapt to the experimental setting, we assume that $1.5b > c > b$, which is a subset of the above reduced form parameters.
% todo: check whether it's n large or relies on infrequent favours
%The game is a reduced form and a basic variant of the original Jackson, Rodriguez-Barraquer, Tan (JRT) model; we explain the key differences in a later section. In our model, the game begins with some initial network, denoted as $g_0$, at time period $t=0$. At any time period $t$, there is a chance that an agent $i$ will be called upon. It is possible that no agent is called upon in any given time period; in fact, the time between periods are small, so that the chance of more than one agent being called upon in the same period goes to 0. When an agent $i$ is called, agent $i$ is then presented the overall network at time $t$ and can choose to delete one link between him and his neighbors, or choose to not delete any links. If agent $i$ deletes with his neighbor, agent $j$, this gives an immediate payoff $c$ to agent $i$ and payoff $0$ to agent $j$. This represents the payoff of not returning a favour. Edge $ij$ is then deleted from the network, and the resultant network is $g_t - ij$. If agent $i$ chooses not to delete any links, no agent gets any immediate payoff, and the resultant network remains as $g_t$. The next agent is then called on at random, at time period $t+1$. Agents are aware of the game, the payoffs and the current network when they make their decision, but they are not aware of the decisions of others and the full history of the network.\\

%This game is an infinite game. If a network $g'$ continues in perpetuity, then each remaining link $ij \in g'$ gives both agents $i$ and $j$ payoff of $b$ each. This represents the present discounted value of a perpetual mutual favour-exchange relationship. Assume that $2b > c > b$.\\


%27/2/21:
% 1. We should have three propositions - 2 from JRT and 1 from us. Clear how proposition maps to the hypothesis.
% 2. We wanted to move towards having a setup of the model that was the Jackson, except for a couple of things. in the design section, to explain how we translate some features of the formal model into our design. Right now, we are presenting the model as deleting links, rather than the Jackson one. Not sure the proof of the Jackson statements are going to go through.
%simplify straightaway in theory:
%% Link formation at the start (doesn't affect results)
%% Limitation of c to 1.5b (because results from Jackson are going to follow through.) CS proposition is going to go through. it's a subset of the proof. Obvious.
%Things in the design:
%% Sequential nature etc
%% Justify them - experimentally and say the theory goes through with this one modification, and proof of that in the Appendix.
% Start by putting things that are now at the end (benefit in the end, machinery model)

%23/3
%1. We should have the three propositions, make sure the language is clear

%\begin{itemize}
%    \item also here we need to be more formal
%    \item let's put "theoremstyle" statements for the key definitions (so Definition 1. etc). we can discuss in the call but i can see we need at least three: transitively critical, social quilt, and cognitively stable
%    \item let's put characterizations as propositions. we need at least 3 propositions for rnp, sq and cs (obviously for the first two no proof is required, maybe we need to show in the appendix how the reduced form model maps to the original one)
%    \item to be discussed: do we need more propositions for cs networks that describe some of their propserties? discuss in the call whether to include them, one corollary that may be worth including is that the triangle is the only network that is both sq and cs
%\end{itemize}

While all damage in a triangle network is "local damage" by definition, for the purposes of analysing individual decisions, we consider the triangle network as a social quilt (since "robustness" describes how the network evolves rather than affect agent behaviour).\\

